Distilling a Geospatial Foundation Model into Compact Surface-Water Segmenters

Geospatial foundation models segment surface water accurately, but their size limits deployment on edge hardware. Therefore, we distill a 300-million-parameter Prithvi-EO-2.0 teacher, fine-tuned on the 252 hand-labeled Sen1Floods11 training images, into compact student models. The teacher labels 2,500 Sentinel-2 images around flood alerts and supervises the students via its labels and probability maps, without manual annotation. A 0.7-million-parameter EfficientViT-B0 student achieves the teacher's accuracy in water intersection over union (IoU) on WorldFloods-v2, STURM-Flood and 97 held-back WorldFloods events. Unlike prior work, we evaluate every model on four test sets from three public datasets and on two new dry-scene sets. Controlled comparisons show that teacher labels achieve human-level annotation quality for student training on the same images. The teacher's probability maps account for much of its value, and the full pipeline adds 5.7 IoU points on the held-back events over training on hand labels alone. All students, with parameter counts ranging from about 1,000 to 32.5 million, perform within 2 IoU points of the teacher on WorldFloods-v2 and STURM-Flood. On a Jetson Xavier NX, the main student runs as a 1.6-megabyte mixed 8-bit integer and 16-bit floating-point engine at 4.9 milliseconds per 512-by-512 image, and a 12,230-parameter student runs in full 8-bit integer format within 0.5 IoU points of its 32-bit version. The main student outperforms a fixed water index by 11.5 IoU points on the held-back events and raises false alarms on under 10\% rather than 57.0\% of water-free windows, as unattended use requires.

==> tables/device_accuracy.tex <==
\rowcolor{useGPU}Main, ReLU6 & mixed INT8/FP16 & +2.0 [+0.3, +3.8] & +0.9 [$-$0.2, +2.3] & $-$1.7 [$-$4.3, +0.3] \\
(deployed) & FP32 $-$ Hardswish FP32 & $-$2.6 [$-$6.8, +0.1] & $-$0.7 [$-$1.9, +0.2] & $-$0.6 [$-$1.1, 0.0] \\
 & mixed INT8/FP16 $-$ Hardswish FP32 & $-$0.6 [$-$4.2, +2.7] & +0.2 [$-$0.7, +1.1] & $-$2.2 [$-$5.0, $-$0.2] \\
\midrule
Main, Hardswish & FP16 & +0.1 [0.0, +0.2] & 0.0 [0.0, +0.1] & 0.0 [0.0, +0.1] \\
 & mixed INT8 & $-$0.6 [$-$2.1, +0.8] & $-$0.5 [$-$1.5, +0.1] & $-$3.3 [$-$5.8, $-$1.2] \\
 & full INT8 & \multicolumn{3}{l}{not possible: the attention needs floating point} \\
\midrule
Tiny student & FP16 & 0.0 [0.0, 0.0] & 0.0 [0.0, 0.0] & 0.0 [0.0, 0.0] \\
 & mixed INT8 & $-$0.3 [$-$0.4, $-$0.1] & $-$0.2 [$-$0.3, $-$0.1] & $-$1.2 [$-$2.1, $-$0.5] \\
\rowcolor{useINT} & full INT8 & 0.0 [$-$0.4, +0.3] & $-$0.1 [$-$0.3, +0.2] & $-$0.5 [$-$1.0, 0.0] \\
\midrule
Micro student & FP16 & 0.0 [0.0, 0.0] & 0.0 [0.0, 0.0] & 0.0 [0.0, 0.0] \\
 & mixed INT8 & +1.2 [+0.1, +2.9] & $-$0.3 [$-$1.0, +0.2] & $-$1.2 [$-$2.2, $-$0.3] \\
 & full INT8 & +1.1 [0.0, +2.8] & $-$0.3 [$-$0.9, +0.1] & $-$1.3 [$-$2.4, $-$0.4] \\


==> tables/device_benchmark.tex <==
Main, ReLU6 & FP32 & 7.22 & 7.33 & 138 & 3.48 & 7.81/8.29 & 1.00 & \textit{73.4} & \textit{79.0} & \textit{49.5} & 4.8 \\
\rowcolor{useGPU}(deployed) & mixed INT8/FP16 & 4.94 & 4.96 & 188 & 1.59 & 5.74/6.49 & 1.46 & +2.0 & +0.9 & $-$1.7 & 9.6 \\
 & full INT8 & \multicolumn{10}{l}{not possible: the attention needs floating point} \\
\midrule
Main, Hardswish & FP32 & 9.38 & 9.55 & 107 & 3.92 & 7.61/7.75 & 1.00 & \textit{76.0} & \textit{79.7} & \textit{50.1} & 5.5 \\
(Table~II weights) & FP16 & 5.96 & 6.02 & 167 & 2.97 & 6.89/7.10 & 1.57 & +0.1 & 0.0 & 0.0 & 5.5 \\
 & mixed INT8/FP32 & 12.26 & 12.33 & 79 & 2.54 & 6.72/6.94 & 0.76 & $-$0.6 & $-$0.5 & $-$3.3 & 5.2 \\
\midrule
Tiny (12,230) & FP32 & 1.75 & 1.98 & 572 & 0.14 & 8.00/8.08 & 1.00 & \textit{78.1} & \textit{79.2} & \textit{48.1} & 7.1 \\
 & FP16 & 1.50 & 1.54 & 663 & 0.45 & 7.78/7.96 & 1.16 & 0.0 & 0.0 & 0.0 & 7.1 \\
 & mixed INT8 & 1.48 & 1.52 & 670 & 0.47 & 6.88/7.02 & 1.18 & $-$0.3 & $-$0.2 & $-$1.2 & 7.1 \\
\rowcolor{useINT} & full INT8 & 1.76 & 1.78 & 568 & 0.56 & 6.84/7.26 & 0.99 & 0.0 & $-$0.1 & $-$0.5 & 7.5 \\
\midrule
Micro (1,266) & FP32 & 1.18 & 1.22 & 843 & 0.07 & 7.75/8.08 & 1.00 & \textit{76.0} & \textit{78.1} & \textit{49.8} & 13.0 \\
 & FP16 & 1.18 & 1.20 & 847 & 0.20 & 7.55/7.71 & 1.00 & 0.0 & 0.0 & 0.0 & 13.0 \\
 & mixed INT8 & 1.19 & 1.20 & 841 & 0.44 & 6.17/6.41 & 1.00 & +1.2 & $-$0.3 & $-$1.2 & 14.0 \\
 & full INT8 & 2.72 & 2.74 & 367 & 0.62 & 6.31/6.86 & 0.44 & +1.1 & $-$0.3 & $-$1.3 & 13.7 \\


==> tables/device_energy.tex <==
Main, ReLU6 & FP32 & --- & 56.4 \\
(deployed) & mixed INT8/FP16 & --- & 30.6 \\
\midrule
Main, Hardswish & FP32 & 143.2 & 71.2 \\
 & FP16 & 85.7 & 41.1 \\
 & mixed INT8 & 169.5 & 85.0 \\
\midrule
Tiny student & FP32 & 27.6 & 14.3 \\
 & FP16 & 22.9 & 11.7 \\
 & mixed INT8 & 21.1 & 10.3 \\
 & full INT8 & 24.2 & 12.1 \\
\midrule
Micro student & FP32 & 17.6 & 9.2 \\
 & FP16 & 17.3 & 8.9 \\
 & mixed INT8 & 15.8 & 7.3 \\
 & full INT8 & 34.4 & 17.2 \\


==> tables/device_optimized_engines.tex <==
Tiny & FP16 control & 1.320 & 1.361 & 756.5 & 0.453 & 8.08/8.12 & 1.00 \\
 & INT8 body + decoder & 1.234 & 1.244 & 810.9 & 0.421 & 7.08/7.18 & 1.07 \\
Micro & FP16 control & 1.035 & 1.051 & 971.2 & 0.202 & 7.87/8.53 & 1.00 \\
 & custom integer CUDA & 0.799 & 0.820 & 1186.7 & -- & 9.32/9.57 & 1.30 \\


==> tables/device_speed_power.tex <==
Main student & FP32 & 9.38 & 9.55 & 106.5 & 3.918 & 7.61 & 7.75 & 1.00 \\
 & FP16 & 5.96 & 6.02 & 167.3 & 2.972 & 6.89 & 7.10 & 1.57 \\
 & mixed INT8 & 12.26 & 12.33 & 79.2 & 2.538 & 6.72 & 6.94 & 0.76 \\
 & full INT8 & \multicolumn{7}{l}{unavailable under validated precision policy} \\
\midrule
Tiny student & FP32 & 1.75 & 1.98 & 571.5 & 0.138 & 8.00 & 8.08 & 1.00 \\
 & FP16 & 1.50 & 1.54 & 663.2 & 0.451 & 7.78 & 7.96 & 1.16 \\
 & mixed INT8 & 1.48 & 1.52 & 670.5 & 0.471 & 6.88 & 7.02 & 1.18 \\
 & full INT8 & 1.76 & 1.78 & 568.3 & 0.561 & 6.84 & 7.26 & 0.99 \\
\midrule
Micro student & FP32 & 1.18 & 1.22 & 843.2 & 0.071 & 7.75 & 8.08 & 1.00 \\
 & FP16 & 1.18 & 1.20 & 846.9 & 0.202 & 7.55 & 7.71 & 1.00 \\
 & mixed INT8 & 1.19 & 1.20 & 840.9 & 0.441 & 6.17 & 6.41 & 1.00 \\
 & full INT8 & 2.72 & 2.74 & 367.0 & 0.621 & 6.31 & 6.86 & 0.44 \\


==> tables/per_pixel_rules.tex <==
Per-pixel rule, 252 hand labels & 79.5 & 78.5 & 37.5 & 57.2 \\
Per-pixel rule, 2,500 teacher labels & 58.1 & 51.1 & 30.6 & 47.5 \\
MNDWI $>0$ & 68.3 & 71.2 & 50.4 & 49.3 \\
Rule (hand labels) $-$ MNDWI & \textbf{+11.1 [+3.6, +18.7]} & +7.3 [0.0, +17.8] & \textbf{$-$12.8 [$-$21.1, $-$5.9]} & \textbf{+7.9 [+5.6, +10.3]} \\


==> tables/pooled_water_iou.tex <==
Teacher & 81.7 & 79.1 & 73.9 & 79.4 & 67.7 & 49.9 \\
MNDWI $>0$ & 65.0 & 68.3 & 74.8 & 71.2 & 67.4 & 50.4 \\
\midrule
Main student & 78.5 & 76.1 & 75.4 & 79.7 & 68.3 & 50.1 \\
Tiny student & 80.6 & 78.1 & 76.5 & 79.2 & 67.3 & 48.1 \\
Micro student & 78.7 & 76.0 & 75.8 & 78.1 & 68.1 & 49.8 \\
Main student, no teacher & 77.5 & 74.8 & 61.5 & 69.6 & 63.4 & 47.2 \\
Main student, with teacher's maps & 78.3 & 75.7 & 67.9 & 74.9 & 67.2 & 50.9 \\
\midrule
MobileNetV3-Small & 79.3 & 77.1 & 75.0 & 79.6 & 69.0 & 51.4 \\
LightFormer-ResNet18 & 78.6 & 75.9 & 73.8 & 78.7 & 68.3 & 49.3 \\
UNet-ResNet50 & 80.9 & 78.2 & 74.7 & 79.3 & 67.4 & 48.5 \\
MobileNetV3-Small, no teacher & 79.0 & 76.8 & 71.9 & 75.1 & 61.1 & 48.3 \\
LightFormer-ResNet18, no teacher & 77.4 & 75.6 & 63.8 & 71.7 & 65.2 & 48.8 \\
LightFormer, authors' setup, no teacher & 80.2 & 78.3 & 75.7 & 78.1 & 67.8 & 50.2 \\
UNet-ResNet50, no teacher & 82.8 & 80.8 & 74.1 & 78.0 & 64.0 & 48.7 \\
Tiny student, no teacher & 83.4 & 81.2 & 76.1 & 79.2 & 62.9 & 45.8 \\
Micro student, no teacher & 82.2 & 80.2 & 77.9 & 79.0 & 68.2 & 50.2 \\


==> tables/student_accuracy.tex <==
Micro student & 1,266 & 252 hand labels, cross-entropy (no teacher) & 80.2 $\pm$ 1.0 & 79.0 $\pm$ 0.7 & 50.2 $\pm$ 0.7 & 58.0 $\pm$ 0.6 & 17.5 \\
 &  & 252 hand labels + teacher's maps & 79.5 $\pm$ 0.8 & 79.0 $\pm$ 0.4 & 48.0 $\pm$ 6.7 & 58.5 $\pm$ 0.6 & 16.2 \\
 &  & teacher labels on the same 252 images & 79.2 $\pm$ 1.0 & 78.8 $\pm$ 0.8 & 45.8 $\pm$ 6.5 & 58.5 $\pm$ 1.0 & 17.0 \\
 &  & 2,500 teacher-labeled GDACS images & 78.3 $\pm$ 1.6 & 78.7 $\pm$ 0.9 & 48.0 $\pm$ 1.6 & 59.4 $\pm$ 1.3 & 12.1 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 77.3 $\pm$ 1.0 & 78.0 $\pm$ 0.7 & 50.4 $\pm$ 0.4 & 58.1 $\pm$ 0.7 & 19.2 \\
\midrule
Tiny student & 12,230 & 252 hand labels, cross-entropy (no teacher) & 81.2 $\pm$ 1.2 & 79.2 $\pm$ 0.8 & 45.8 $\pm$ 5.6 & 59.3 $\pm$ 0.5 & 11.2 \\
 &  & 252 hand labels + teacher's maps & 81.5 $\pm$ 0.7 & 79.2 $\pm$ 0.6 & 47.4 $\pm$ 1.9 & 59.1 $\pm$ 0.7 & 8.5 \\
 &  & teacher labels on the same 252 images & 80.6 $\pm$ 1.0 & 79.5 $\pm$ 0.4 & 44.4 $\pm$ 7.1 & 60.0 $\pm$ 0.1 & 9.0 \\
 &  & 2,500 teacher-labeled GDACS images & 80.2 $\pm$ 0.2 & 79.8 $\pm$ 0.2 & 48.0 $\pm$ 1.2 & 60.8 $\pm$ 0.7 & 5.9 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 79.6 $\pm$ 0.3 & 79.4 $\pm$ 0.2 & 48.8 $\pm$ 1.4 & 60.7 $\pm$ 0.2 & 4.3 \\
\midrule
EfficientViT-B0 & 0.7\,M & 252 hand labels, cross-entropy (no teacher) & 74.8 $\pm$ 1.7 & 69.6 $\pm$ 3.9 & 47.2 $\pm$ 1.5 & 55.1 $\pm$ 1.2 & 11.8 \\
 &  & 252 hand labels + teacher's maps & 75.1 $\pm$ 1.3 & 74.0 $\pm$ 2.6 & 50.1 $\pm$ 1.2 & 57.3 $\pm$ 1.1 & 6.3 \\
 &  & teacher labels on the same 252 images & 75.2 $\pm$ 0.7 & 69.8 $\pm$ 2.1 & 46.1 $\pm$ 1.3 & 55.2 $\pm$ 1.6 & 9.4 \\
 &  & 2,500 teacher-labeled GDACS images & 75.5 $\pm$ 1.2 & 78.8 $\pm$ 1.4 & 48.2 $\pm$ 0.8 & 60.9 $\pm$ 0.2 & 10.6 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 76.1 $\pm$ 0.8 & 79.9 $\pm$ 0.5 & 50.3 $\pm$ 0.4 & 60.9 $\pm$ 0.5 & 7.7 \\
\midrule
MobileNetV3-Small & 3.55\,M & 252 hand labels, cross-entropy (no teacher) & 76.8 $\pm$ 1.2 & 75.1 $\pm$ 1.4 & 48.3 $\pm$ 3.5 & 55.1 $\pm$ 0.5 & 15.6 \\
 &  & 252 hand labels + teacher's maps & 77.6 $\pm$ 1.3 & 77.9 $\pm$ 0.1 & 52.0 $\pm$ 0.7 & 56.8 $\pm$ 0.2 & 13.5 \\
 &  & teacher labels on the same 252 images & 76.8 $\pm$ 0.7 & 75.2 $\pm$ 0.6 & 50.8 $\pm$ 1.1 & 56.1 $\pm$ 0.4 & 17.2 \\
 &  & 2,500 teacher-labeled GDACS images & 76.2 $\pm$ 0.3 & 77.8 $\pm$ 1.0 & 49.7 $\pm$ 0.4 & 60.9 $\pm$ 0.2 & 5.9 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 76.6 $\pm$ 0.2 & 79.3 $\pm$ 0.3 & 51.3 $\pm$ 0.2 & 60.5 $\pm$ 0.4 & 3.4 \\
\midrule
LightFormer-ResNet18 & 11.43\,M & 252 hand labels, cross-entropy (no teacher) & 75.6 $\pm$ 0.7 & 71.7 $\pm$ 0.4 & 48.8 $\pm$ 0.7 & 55.9 $\pm$ 0.7 & 11.0 \\
 &  & 252 hand labels + teacher's maps & 76.3 $\pm$ 1.8 & 73.8 $\pm$ 0.9 & 50.9 $\pm$ 0.7 & 57.3 $\pm$ 1.3 & 6.2 \\
 &  & teacher labels on the same 252 images & 75.1 $\pm$ 1.2 & 72.6 $\pm$ 0.8 & 48.9 $\pm$ 0.9 & 55.7 $\pm$ 1.3 & 7.8 \\
 &  & 2,500 teacher-labeled GDACS images & 74.4 $\pm$ 2.1 & 76.9 $\pm$ 2.5 & 44.9 $\pm$ 1.5 & 59.9 $\pm$ 0.2 & 17.0 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 75.6 $\pm$ 1.4 & 77.9 $\pm$ 0.6 & 48.6 $\pm$ 0.8 & 59.9 $\pm$ 0.4 & 14.3 \\
 &  & authors' setup, 252 hand labels & 78.3 $\pm$ 1.0 & 78.1 $\pm$ 1.9 & 50.2 $\pm$ 2.6 & 57.9 $\pm$ 0.2 & 11.1 \\
 &  & authors' setup, 2,500 teacher labels & 76.9 $\pm$ 1.0 & 77.8 $\pm$ 1.8 & 48.3 $\pm$ 2.2 & 61.5 $\pm$ 0.4 & 7.9 \\
\midrule
UNet-ResNet50 & 32.5\,M & 252 hand labels, cross-entropy (no teacher) & 80.8 $\pm$ 0.3 & 78.0 $\pm$ 0.9 & 48.7 $\pm$ 1.5 & 56.9 $\pm$ 0.5 & 9.9 \\
 &  & 252 hand labels + teacher's maps & 79.7 $\pm$ 0.9 & 79.9 $\pm$ 0.5 & 50.8 $\pm$ 0.4 & 58.7 $\pm$ 0.6 & 5.0 \\
 &  & teacher labels on the same 252 images & 79.6 $\pm$ 0.9 & 77.9 $\pm$ 0.9 & 50.0 $\pm$ 1.6 & 58.3 $\pm$ 0.8 & 10.7 \\
 &  & 2,500 teacher-labeled GDACS images & 77.9 $\pm$ 0.7 & 77.7 $\pm$ 1.0 & 47.6 $\pm$ 0.7 & 61.1 $\pm$ 0.2 & 2.9 \\
\rowcolor{rowhl} &  & 2,500 teacher-labeled images + maps & 78.2 $\pm$ 1.4 & 79.9 $\pm$ 0.3 & 47.9 $\pm$ 0.8 & 61.6 $\pm$ 0.1 & 2.8 \\


==> tables/student_designs.tex <==
EfficientViT-B0 & 0.7\,M & labels only & 74.7 $\pm$ 1.0 & 78.4 $\pm$ 0.9 & 47.5 $\pm$ 2.2 \\
 &  & logit distillation & 76.1 $\pm$ 0.6 & 79.7 $\pm$ 0.2 & \textbf{50.1} $\pm$ 0.8 \\
 &  & OFA & \textbf{76.3} $\pm$ 1.0 & \textbf{79.9} $\pm$ 0.2 & 49.5 $\pm$ 0.7 \\
\midrule
MobileNetV3-Small & 3.55\,M & labels only & \textbf{77.1} $\pm$ 1.3 & 78.3 $\pm$ 1.4 & 48.7 $\pm$ 0.7 \\
 &  & logit distillation & \textbf{77.1} $\pm$ 0.6 & 79.6 $\pm$ 0.2 & 51.4 $\pm$ 0.3 \\
 &  & OFA & 76.7 $\pm$ 0.9 & \textbf{79.8} $\pm$ 0.3 & \textbf{51.6} $\pm$ 0.5 \\
\midrule
LightFormer-ResNet18 & 11.43\,M & labels only & 75.0 $\pm$ 1.4 & 75.6 $\pm$ 2.5 & 45.0 $\pm$ 1.5 \\
 &  & logit distillation & 75.9 $\pm$ 1.3 & 78.7 $\pm$ 0.6 & \textbf{49.3} $\pm$ 1.1 \\
 &  & OFA & \textbf{76.7} $\pm$ 0.6 & \textbf{78.9} $\pm$ 0.3 & 49.0 $\pm$ 0.7 \\


==> tables/student_differences.tex <==
Micro student & maps on the 252 hand-labeled images & $-$0.7 [$-$1.6, +0.1] & 0.0 [$-$0.6, +0.8] & \textbf{$-$2.1 [$-$4.0, $-$0.6]} & \textbf{+0.5 [+0.2, +0.9]} \\
 & teacher $-$ human labels, same 252 images & \textbf{$-$1.0 [$-$1.8, $-$0.3]} & $-$0.2 [$-$0.7, +0.5] & \textbf{$-$4.4 [$-$6.9, $-$2.3]} & \textbf{+0.5 [+0.2, +0.9]} \\
 & teacher pipeline $-$ hand labels alone & \textbf{$-$2.9 [$-$4.4, $-$1.7]} & $-$1.0 [$-$2.3, +0.2] & +0.2 [$-$0.8, +1.3] & +0.1 [$-$0.7, +0.9] \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & \textbf{$-$2.2 [$-$3.0, $-$1.5]} & $-$1.0 [$-$2.4, +0.2] & \textbf{+2.4 [+0.6, +4.4]} & $-$0.4 [$-$1.1, +0.3] \\
 & maps on the 2,500 teacher-labeled images & \textbf{$-$1.0 [$-$1.6, $-$0.3]} & \textbf{$-$0.8 [$-$1.6, $-$0.1]} & \textbf{+2.4 [+0.8, +4.3]} & \textbf{$-$1.3 [$-$1.6, $-$0.9]} \\
\midrule
Tiny student & maps on the 252 hand-labeled images & +0.4 [$-$0.3, +1.2] & 0.0 [$-$0.6, +0.6] & \textbf{+1.6 [+0.6, +2.8]} & $-$0.1 [$-$0.5, +0.2] \\
 & teacher $-$ human labels, same 252 images & $-$0.5 [$-$1.4, +0.6] & +0.3 [$-$0.4, +1.0] & $-$1.4 [$-$3.6, +0.3] & \textbf{+0.7 [+0.3, +1.2]} \\
 & teacher pipeline $-$ hand labels alone & $-$1.5 [$-$2.9, 0.0] & +0.2 [$-$1.3, +1.5] & \textbf{+3.0 [+0.7, +5.5]} & \textbf{+1.4 [+0.6, +2.3]} \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & \textbf{$-$1.9 [$-$2.9, $-$0.9]} & +0.2 [$-$1.1, +1.6] & +1.4 [$-$0.4, +3.3] & \textbf{+1.5 [+0.7, +2.5]} \\
 & maps on the 2,500 teacher-labeled images & $-$0.6 [$-$1.3, +0.1] & $-$0.4 [$-$0.8, 0.0] & +0.8 [$-$0.4, +2.3] & $-$0.1 [$-$0.5, +0.3] \\
\midrule
EfficientViT-B0 & maps on the 252 hand-labeled images & +0.2 [$-$0.2, +0.7] & \textbf{+4.4 [+1.7, +7.2]} & \textbf{+2.9 [+1.4, +4.5]} & \textbf{+2.2 [+1.4, +3.1]} \\
 & teacher $-$ human labels, same 252 images & +0.4 [$-$0.3, +1.5] & +0.2 [$-$3.9, +3.2] & $-$1.1 [$-$2.4, +0.4] & +0.2 [$-$0.9, +1.0] \\
 & teacher pipeline $-$ hand labels alone & +1.3 [$-$1.4, +4.2] & \textbf{+10.3 [+3.1, +20.7]} & \textbf{+3.2 [+0.2, +6.4]} & \textbf{+5.8 [+4.2, +7.8]} \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & +1.0 [$-$1.4, +3.7] & \textbf{+5.9 [+0.9, +15.1]} & +0.2 [$-$2.5, +3.1] & \textbf{+3.6 [+2.2, +5.2]} \\
 & maps on the 2,500 teacher-labeled images & +0.6 [$-$0.7, +2.0] & +1.1 [$-$0.4, +3.5] & \textbf{+2.1 [+0.6, +4.6]} & 0.0 [$-$0.3, +0.3] \\
\midrule
MobileNetV3-Small & maps on the 252 hand-labeled images & +0.8 [$-$0.5, +2.2] & \textbf{+2.9 [+1.3, +4.7]} & \textbf{+3.7 [+1.9, +5.9]} & \textbf{+1.7 [+1.2, +2.1]} \\
 & teacher $-$ human labels, same 252 images & 0.0 [$-$1.0, +1.0] & +0.1 [$-$1.6, +1.4] & \textbf{+2.5 [+1.1, +4.2]} & \textbf{+1.0 [+0.6, +1.4]} \\
 & teacher pipeline $-$ hand labels alone & $-$0.3 [$-$4.7, +3.3] & \textbf{+4.3 [+1.6, +7.6]} & \textbf{+3.0 [+0.6, +5.8]} & \textbf{+5.4 [+3.7, +7.6]} \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & $-$1.1 [$-$4.7, +2.3] & \textbf{+1.4 [+0.2, +3.0]} & $-$0.7 [$-$2.3, +0.6] & \textbf{+3.7 [+2.3, +5.6]} \\
 & maps on the 2,500 teacher-labeled images & +0.3 [$-$0.4, +1.3] & +1.5 [$-$0.5, +5.0] & \textbf{+1.6 [+0.3, +3.6]} & $-$0.4 [$-$0.9, 0.0] \\
\midrule
LightFormer-ResNet18 & maps on the 252 hand-labeled images & +0.7 [$-$0.6, +2.5] & \textbf{+2.1 [+0.1, +5.4]} & \textbf{+2.1 [+0.1, +4.8]} & \textbf{+1.4 [+0.7, +2.2]} \\
 & teacher $-$ human labels, same 252 images & $-$0.4 [$-$1.2, +0.4] & +0.9 [$-$0.4, +2.7] & +0.2 [$-$1.0, +1.3] & $-$0.3 [$-$1.6, +1.2] \\
 & teacher pipeline $-$ hand labels alone & 0.0 [$-$3.0, +3.4] & +6.2 [0.0, +17.5] & $-$0.2 [$-$2.8, +2.6] & \textbf{+4.0 [+2.5, +5.9]} \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & $-$0.7 [$-$2.6, +1.2] & +4.1 [$-$0.5, +12.4] & \textbf{$-$2.3 [$-$4.3, $-$0.5]} & \textbf{+2.6 [+1.6, +3.9]} \\
 & maps on the 2,500 teacher-labeled images & +1.2 [$-$0.5, +3.4] & +1.1 [$-$0.4, +2.8] & \textbf{+3.7 [+1.3, +6.9]} & +0.1 [$-$0.2, +0.4] \\
 & authors' $-$ common setup, 252 hand labels & +2.7 [$-$0.2, +6.0] & +6.3 [$-$0.4, +18.4] & +1.4 [$-$1.3, +4.7] & \textbf{+1.9 [+0.2, +4.0]} \\
 & authors' $-$ common setup, 2,500 teacher labels & \textbf{+2.5 [+0.5, +4.7]} & +0.9 [$-$0.3, +2.2] & \textbf{+3.4 [+0.5, +7.1]} & \textbf{+1.6 [+0.8, +2.5]} \\
\midrule
UNet-ResNet50 & maps on the 252 hand-labeled images & $-$1.1 [$-$2.8, +0.1] & \textbf{+1.8 [+0.5, +3.7]} & +2.1 [$-$0.3, +5.0] & \textbf{+1.8 [+1.1, +2.6]} \\
 & teacher $-$ human labels, same 252 images & $-$1.1 [$-$2.5, +0.6] & $-$0.1 [$-$0.4, +0.2] & \textbf{+1.3 [+0.1, +2.7]} & \textbf{+1.4 [+0.5, +2.6]} \\
 & teacher pipeline $-$ hand labels alone & $-$2.6 [$-$5.7, +1.6] & +1.9 [$-$0.1, +5.1] & $-$0.8 [$-$4.9, +3.5] & \textbf{+4.7 [+3.1, +6.8]} \\
 & 2,500 teacher-labeled $-$ 252 hand-labeled, both with maps & $-$1.5 [$-$4.1, +2.1] & +0.1 [$-$1.3, +1.9] & \textbf{$-$2.9 [$-$6.3, $-$0.2]} & \textbf{+2.9 [+1.7, +4.4]} \\
 & maps on the 2,500 teacher-labeled images & +0.2 [$-$0.9, +1.3] & \textbf{+2.3 [+0.1, +6.3]} & +0.4 [$-$0.8, +1.6] & \textbf{+0.5 [+0.1, +1.0]} \\


==> tables/submitted_vs_revised.tex <==
Teacher & STURM-Flood & 75.4 & 76.6 & 49.9 \\
Teacher & WorldFloods & 77.2 & 81.5 & 79.4 \\
MNDWI $>0$ & STURM-Flood & 74.7 & 76.0 & 50.4 \\
MNDWI $>0$ & WorldFloods & 75.9 & 81.4 & 71.2 \\
Earlier student & STURM-Flood & 76.0 & 77.3 & 50.3 \\
Earlier student & WorldFloods & 77.1 & 82.7 & 79.5 \\


==> tables/water_indices.tex <==
MNDWI, threshold 0 & 68.3 & 71.2 & 50.4 & 49.3 & 57.0 \\
MNDWI, tuned on S11 & 76.4 & 73.9 & 42.8 & 53.3 & 38.3 \\
NDWI, threshold 0 & 67.4 & 66.0 & 45.8 & 53.7 & \textbf{14.8} \\
NDWI, tuned on S11 & 76.3 & 70.1 & 49.8 & 54.3 & 31.9 \\
AWEI$_\text{nsh}$, threshold 0 & 76.1 & 73.5 & 30.9 & 52.4 & 21.6 \\
AWEI$_\text{nsh}$, tuned on S11 & 74.2 & 73.8 & 29.6 & 52.5 & 20.4 \\
AWEI$_\text{sh}$, threshold 0 & 76.8 & 73.9 & 51.8 & 53.6 & 44.2 \\
AWEI$_\text{sh}$, tuned on S11 & 79.0 & 76.6 & 45.5 & 55.8 & 28.8 \\
WI2015, threshold 0 & 75.1 & 73.2 & \textbf{52.0} & 52.4 & 55.5 \\
WI2015, tuned on S11 & \textbf{79.5} & \textbf{77.4} & 45.3 & \textbf{56.6} & 28.0 \\
\midrule
Teacher & 79.1 & 79.4 & 49.9 & 60.7 & 1.5 \\
Main student & 76.1 & 79.7 & 50.1 & 60.8 & 5.4 \\
Tiny student & 78.1 & 79.2 & 48.1 & 60.0 & 7.1 \\


==> tables/water_iou_measures.tex <==
Teacher & S11 test & 89.7 & 89.5 & 81.7 & 79.1 \\
 & WorldFloods test & 77.1 & 81.5 & 73.9 & 79.4 \\
 & STURM-Flood & 75.5 & 76.6 & 67.7 & 49.9 \\
\midrule
Main student & S11 test & 87.7 & 87.6 & 78.5 & 76.1 \\
 & WorldFloods test & 76.4 & 82.5 & 75.4 & 79.7 \\
 & STURM-Flood & 75.6 & 77.2 & 68.3 & 50.1 \\
\midrule
MNDWI $>0$ & S11 test & 78.9 & 78.9 & 65.0 & 68.3 \\
 & WorldFloods test & 76.3 & 81.4 & 74.8 & 71.2 \\
 & STURM-Flood & 74.7 & 76.0 & 67.4 & 50.4 \\

